To what extent can we analyze Kotlin programs using existing Java taint analysis tools? (Extended Version)

As an alternative to Java, Kotlin has gained rapid popularity since its introduction and has become the default choice for developing Android apps. However, due to its interoperability with Java, Kotlin programs may contain almost the same security vulnerabilities as their Java counterparts. Hence, we question: to what extent can one use an existing Java static taint analysis on Kotlin code? In this paper, we investigate the challenges in implementing a taint analysis for Kotlin compared to Java. To answer this question, we performed an exploratory study where each Kotlin construct was examined and compared to its Java equivalent. We identified 18 engineering challenges that static-analysis writers need to handle differently due to Kotlin's unique constructs or the differences in the generated bytecode between the Kotlin and Java compilers. For eight of them, we provide a conceptual solution, while six of those we implemented as part of SecuCheck-Kotlin, an extension to the existing Java taint analysis SecuCheck.

==> additional.tex <==
\section{Additional found problems}
\label{sec:additional}

Explain the remaining problems we found in short. May be give two tables which dont have any problem and another table for the features associated with some problems (Like in my thesis).

==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

Evaluation, Two research questions and a table

==> extensions.tex <==
\section{Extensions}
\label{sec:extensions}

Briefly explain all the extension that we added. Explain neatly what are the problems and how we solved.

\rk{Discuss about the problems that we found but not extended in \secucheckkotlin}

==> foundations.tex <==
\section{Overview / \secucheck}
\label{sec:overview}

Talk little about overview of \secucheckkotlin and say it extended from the \secucheck \cite{secucheck} to support taint analysis for Kotlin. And then say we did not change the architecture of \secucheck. May be make it methodology

==> motivation.tex <==
\section{Requirements (0.5 page)}
\label{sec:motivation}


